Zero-Shot Hierarchical Classification on the Common Procurement Vocabulary Taxonomy

Classifying public tenders is a useful task for both companies that are invited to participate and for inspecting fraudulent activities. To facilitate the task for both participants and public administrations, the European Union presented a common taxonomy (Common Procurement Vocabulary, CPV) which is mandatory for tenders of certain importance; however, the contracts in which a CPV label is mandatory are the minority compared to all the Public Administrations activities. Classifying over a real-world taxonomy introduces some difficulties that can not be ignored. First of all, some fine-grained classes have an insufficient (if any) number of observations in the training set, while other classes are far more frequent (even thousands of times) than the average. To overcome those difficulties, we present a zero-shot approach, based on a pre-trained language model that relies only on label description and respects the label taxonomy. To train our proposed model, we used industrial data, which comes from contrattipubblici.org, a service by SpazioDati s.r.l. that collects public contracts stipulated in Italy in the last 25 years. Results show that the proposed model achieves better performance in classifying low-frequent classes compared to three different baselines, and is also able to predict never-seen classes.

==> acm_authors.tex <==
\title{Zero-Shot Hierarchical Classification on the Common Procurement Vocabulary Taxonomy}

% AUTHORS
\author{Federico Moiraghi}
\email{federico.moiraghimotta@unimib.it}
\affiliation{
    \institution{University of Milano Bicocca}}
\email{moiraghi@spaziodati.eu}
\affiliation{
    \institution{SpazioDati s.r.l.}
    \country{Italy}}
\orcid{0000-0002-4613-8115}

\author{Matteo Palmonari}
\email{matteo.palmonari@unimib.it}
\affiliation{
    \institution{University of Milano Bicocca}
    \country{Italy}}
\orcid{0000-0002-1801-5118}

\author{Davide Allavena}
\email{davide.allavena@spaziodati.eu}
\affiliation{
    \institution{SpazioDati s.r.l.}
    \country{Italy}}

\author{Federico Morando}
\email{federico.morando@spaziodati.eu}
\affiliation{
    \institution{SpazioDati s.r.l.}
    \country{Italy}}
% \orcid{0000-0003-1385-2088}

\renewcommand{\shortauthors}{Moiraghi, et al.}


% copyright (TODO)
% \setcopyright{acmcopyright}
% \copyrightyear{2024}
% \acmYear{2024}
% \acmDOI{XXXXXXX.XXXXXXX}  %TODO
% \acmConference[TWC]{TheWebConf2024}{June 03--05, 2018}{Woodstock, NY} %TODO
% \acmPrice{15.00}
% \acmISBN{978-1-4503-XXXX-X/18/06}

  
% OTHER
\begin{CCSXML}
<ccs2012>
   <concept>
       <concept_id>10010147.10010178.10010179.10003352</concept_id>
       <concept_desc>Computing methodologies~Information extraction</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
 </ccs2012>
\end{CCSXML}

\ccsdesc[500]{Computing methodologies~Information extraction}

\keywords{
    hierarchical classification,
    zero-shot,
    common procurement vocabulary,
    taxonomy classification,
    document classification}

\bibliographystyle{ACM-Reference-Format}

==> domande_aperte.tex <==
- premessa:

-- encoding dell'input 
---- BERT 
---- ---- deep fine-tuning (A)
---- ---- non fine-tuned
---- TFIDF+SVD

-- inferenza (scoring, candidate selection, decision)
---- ---- [iterative top-down with sentence classification] score(sentence classification*) with iterative exploration of candidates until some candidates with scores over a certain threshold are found and some confidence constraints are satisfied [iterative top-down] 
-- scoring = sentence classification with fine-tuned BERT
-- candidate selection = top-down exploration with constraints on candidate scores
-- decision = argmax 

{it is based on the iterative exploration of the hierarchy of labels, where at each step, a classification score is computed for all the children of the expanded nodes}
{single-label, and, in particular, where each input is associated with the best label in the hierarchy, independently from its depth}{modification to a multi-label problem --> future work}

---- ---- [iterative top-down with vector classification]


- baseline
-- preso dalla letteratura?
--- 



* sentence classification = classifier(maxpool(tokens(s)))


-- scoring = sentence classification with native BERT
-- candidate selection = top-down exploration with constraints on candidate scores
-- decision = argmax 


--- scoring:
1 ---- sentence classification with fine-tuned BERT (all data with special tokens) [A OK]
------ fine-tuned

(2 ---- sentence classification with native BERT (description only) [B NO] 
------ not fine-tuned
------ fine-tuned)

3 ---- sentence classification with native BERT (all data as plain text) [B NO]
------ not fine-tuned (-)
------ fine-tuned (+)

4 ---- RF on TFIDF+SVD [B OK]
------ one binary classifier for each branch (BL-C) 
------ one binary classifier for each class (NL-C) (+)

--- candidate selection
- iterative top-down: top-down three search with constraints on candidate scores
- all labels: no selection 

--- decision
- best score



- top-down = top-down exploration with RF on TFIDF+SVD (Branch-level classifier)
- per-node = top-down exploration with RF on TFIDF+SVD (Node-level classifier)
- big bang = all labels with RF on TFIDF+SVD (One classifier)

Varie baselines
- RF top-down
- RF per-node
- RF big bang

Tuo approccio (contributor original)
- FT-BSC top-down
  

Ablation studies 
- FT-BSC (plain text / no data separators) top-down 
- RF + FT-BSC top-down
- - cosa succede se si modifica la threshold? > variazioni della the
- - cosa succede si si usa solo threshold?  


- Ci soon altri paper che hanno usato l'approccio sentence classification basato su BERT per classificazione gerarchica di brevi tesi? Importante discutere bene differenza con [4]

- Tipicamente il cross-encoder è applicator dopo un dense retriever (BLINK?) 
--- non abbiamo descrizione... abbiamo solo label
--- come combinare con struttura gerarchica 
------ dense retrieval dei candidati > top 100 (?) > cross-encoder
-- perchè no in question paper? Perchè ci ispiriamo alla letteratura su classificazione gerarchica che suggerisce una esplorazione iterativa 

- Stopping strategy > utili sia score sia "confidence"








